Be Aware of Your Leaders

Advances in blockchains have influenced the State-Machine-Replication (SMR) world and many state-of-the-art blockchain-SMR solutions are based on two pillars: Chaining and Leader-rotation. A predetermined round-robin mechanism used for Leader-rotation, however, has an undesirable behavior: crashed parties become designated leaders infinitely often, slowing down overall system performance. In this paper, we provide a new Leader-Aware SMR framework that, among other desirable properties, formalizes a Leader-utilization requirement that bounds the number of rounds whose leaders are faulty in crash-only executions. We introduce Carousel, a novel, reputation-based Leader-rotation solution to achieve Leader-Aware SMR. The challenge in adaptive Leader-rotation is that it cannot rely on consensus to determine a leader, since consensus itself needs a leader. Carousel uses the available on-chain information to determine a leader locally and achieves Liveness despite this difficulty. A HotStuff implementation fitted with Carousel demonstrates drastic performance improvements: it increases throughput over 2x in faultless settings and provided a 20x throughput increase and 5x latency reduction in the presence of faults.

==> sections/related.tex <==
\section{Related Work \sasha{Should we call it Orthogonal work?:)}}

Orthogonally to more efficient Leader-rotation schemes, there are a number of potential approaches to improve performance of leader-based consensus protocols. 
%
These approaches include state sharding~\cite{chainspace, omniledger, rapidchain, sok-sharding}, layer-two protocols~\cite{sok-layer2, poon2016bitcoin, fastpay, brick}, and efficient transaction dissemination techniques~\cite{narwhal, ozisik2019graphene}. 
%
The key idea of state sharding is to create groups (or shards) of nodes that handle only a subset of all transactions and system state, relying on classical BFT protocols for reaching \emph{intra-shard consensus}~\cite{sok-consensus}. Layer-two protocols enable clients to process off-chain transactions through private communications rather than through the main chain, thus alleviating the load on the main chain. Efficient data-sharing designs decouple the problem of transaction dissemination from consensus. They first disseminate batches of transactions and then reach consensus on short references to these batches, thus alleviating most of the complexity from the consensus protocol.
%
Finally, Mir-BFT~\cite{mir-bft} removes the single-leader bandwidth bottleneck. It allows multiple leaders to propose transaction batches in parallel while avoiding transactions duplication. This technique is proven incredibly effective even for large party sets. Impressively, Mir-BFT's throughput decreases only slowly for large sets up to 100 parties.
%
%Our leader election scheme can obviously be composed with any of the techniques mentioned in this section.
